Red-Teaming for Inducing Societal Bias in Large Language Models

Ensuring the safe deployment of AI systems is critical in industry settings where biased outputs can lead to significant operational, reputational, and regulatory risks. Thorough evaluation before deployment is essential to prevent these hazards. Red-teaming addresses this need by employing adversarial attacks to develop guardrails that detect and reject biased or harmful queries, enabling models to be retrained or steered away from harmful outputs. However, most red-teaming efforts focus on harmful or unethical instructions rather than addressing social bias, leaving this critical area under-explored despite its significant real-world impact, especially in customer-facing systems. We propose two bias-specific red-teaming methods, Emotional Bias Probe (EBP) and BiasKG, to evaluate how standard safety measures for harmful content affect bias. For BiasKG, we refactor natural language stereotypes into a knowledge graph. We use these attacking strategies to induce biased responses from several open- and closed-source language models. Unlike prior work, these methods specifically target social bias. We find our method increases bias in all models, even those trained with safety guardrails. Our work emphasizes uncovering societal bias in LLMs through rigorous evaluation, and recommends measures ensure AI safety in high-stakes industry deployments.

==> results_old.tex <==
\section{Results and Discussion}

\begin{table*}[t]
	
	\renewcommand\arraystretch{0.9}
	
	% \small
	
	\centering
	\setlength{\tabcolsep}{4pt}
	
	\resizebox{0.9\linewidth}{!}{
		
		\begin{tabular}{p{1.5cm}|p{4cm}||ccc|ccc|ccc|ccc|ccc|ccc}
			
			\toprule
			
			\multirow{3}{*}{Dataset} & Model & \multicolumn{6}{c|}{\texttt{Llama3-8b}}&\multicolumn{6}{c|}{\texttt{Llama3-70b}}&\multicolumn{6}{c}{\texttt{Mistral-7b}}\\
			\cmidrule{2-20}
			&Explanation? & \multicolumn{3}{c|}{Y}&\multicolumn{3}{c|}{N}& \multicolumn{3}{c|}{Y}&\multicolumn{3}{c|}{N}& \multicolumn{3}{c|}{Y}&\multicolumn{3}{c}{N}\\
			\cmidrule{2-20}
			&Metric & BR$\uparrow$& RFL $\downarrow$ & NM$\downarrow$ & BR$\uparrow$& RFL $\downarrow$ & NM$\downarrow$ &BR$\uparrow$& RFL $\downarrow$ & NM$\downarrow$ & BR$\uparrow$& RFL $\downarrow$ & NM$\downarrow$ &BR$\uparrow$& RFL $\downarrow$ & NM$\downarrow$ & BR$\uparrow$& RFL $\downarrow$ & NM$\downarrow$ \\
			
			\midrule
			\multirow{3}{*}{BBQ} & EP &  15.7 & 50.5 & 0.0 & 26.3 & 26.0 & 0.1 & 14.7 & 9.6 & 0.1 & 23.2 & 3.3 & 0.0 & 39.1 & 0.4 & 0.1  & 39.6 & 0.3 & 0.2 \\
			&EP + ES & 11.6 & 65.8 & 0.2 & 21.1 & 41.0 & 0.1  & 18.6 & 7.4 & 0.1 & 26.5 & 2.1 & 0.1 & 43.6 & 0.0 & 0.1 & 41.8 & 0.7 & 0.1\\
			&EP + ES + BiasKG & 0.2 & 97.6 & 1.8 & 0.3 & 98.4 & 0.0  & 18.6 & 34.8 & 0.1 & 19.2 & 31.4 & 0.1 & - & - & - & - \\
            \midrule
			\multirow{3}{*}{DTS} &EP & 10.1 & 74.5 & 0.0 & 23.7 & 45.1 & 0.0& 67.3 & 23.3 & 0.0 & 65.0 & 18.1 & 0.0 & 3.0 & 0.0 & 0.0 &2.0 & 0.3 & 0.0 \\
			&EP + ES & 28.8 & 66.7 & 0.0 & 29.0 & 58.2 & 0.0 & 49.5 & 42.8 & 0.0 & 63.0 & 20.4 & 0.0 & 2.8 & 0.1 & 0.1 & 19.4 & 0.0 & 0.0 \\
			&EP + ES + BiasKG & 41.1 & 56.5 & 0.0 & 70.7 & 23.6 & 0.0 & 65.9 & 28.4 & 4.1 & 71.4 & 26.5 & 0.0 & - & - & - & - \\
			\bottomrule
			
		\end{tabular}
		
	}
	
	\caption{Iteratively combining explicit prompting (EP), emotional stimuli (ES), and BiasKG attacks can have varied results depending on model and dataset. We do not report results on the full combination with \texttt{Mistral-7b} as the attack was not effective in our initial experiments.}
	
	\label{tab:combos}
	
	
	%%%
	
\end{table*}

\paragraph{Efficacy of individual attacks.} Our experiment results for individual attacks are summarized in Table \ref{tab:baseline}. We compare all methods to a baseline with our system prompt and no adversarial prompts. \textit{With} explanations refers to experiments where we prompt the model to output an explanation, and \textit{without} explanations is the case where we do not.

Overall, explicit prompting is the most effective at eliciting bias on the BBQ dataset, consistently scoring the highest bias rate across all models (\emph{except} \texttt{GPT-4o}). Our novel BiasKG method is most effective on larger models; it outperforms explicit prompting for \texttt{GPT-4o} and is equivalent for \texttt{Llama3-70b}. For \texttt{Mistral-7b}, the BiasKG method is almost unchanged from the baseline. \texttt{Llama3-8b} sees some slight increase (+2.5\% with explanation and +9.2\% without), but the explicit prompting is still more effective. 


For the DTS dataset, the emotional stimuli and BiasKG methods become more effective --- BiasKG is especially effective on the Llama3 suite of models. For \texttt{Llama3-8b}, the bias rate increases by 35-38\%, while for Llama3-70b it increases by 30-50\%, all without increasing the No Match Rate. This is somewhat expected, as DTS is directly targeting stereotypes that would be found in our bias knowledge graph, while BiasKG is more reliant on the input context and reasoning ability of the LLM. 




The full results for the emotional stimuli experiments can be found in Table \ref{tab:stim}. Overall, for the BBQ dataset, there is no consistent pattern in which scenarios produce higher BR than the others. The largest range between the maximum and minimum BR across the five scenarios tested was observed in \texttt{GPT-3.5-turbo}, with a difference of 13.3\%, while the lowest was with \texttt{Mistral-7b} with 5.6\%. For the DTS dataset, it is interesting to note that asking for an explanation fron \texttt{GPT-3.5-turbo} increases the bias significantly, with a maximum of 96.9\% BR (+38.5\%, compared to without asking for an explanation.) \texttt{GPT-3.5-turbo} also observes the largest range in BR across the five scenarios, ranging from 1.6\% to 96.9\%. This demonstrates the brittleness of safety fine-tuning, further discussed below.


% Our experiment results are summarized in Table \ref{tab:baseline}. Overall, we observe an increase in Deception rate for all models after the application of our BiasKG except for the \texttt{Llama-2} suite of models. The most significant change was seen in \texttt{GPT-4}, where the deception rate increased from 1.5\% to 7.0\%, almost tripling the deception rate. \texttt{Mistral-7b} model, which increased from 36.3\% to 59.7\%. 
% It seems that models better trained to follow instructions are more susceptible to persuasion when presented with Superior Knowledge.

% We also find the No Match rate is high for some models (eg. \texttt{Llama2-13b}) despite incorporating retries and multiple runs. After manual inspection of the generations, the majority of these errors appear to be \emph{refusals} such as ``I cannot make any assumptions about the individuals based on their background or demographic information...'' The No Match rate generally decreases for the Llama 2 models when we ask for an explanation, indicating the BiasKG effectively bypasses guardrails not does not necessarily increase the model's bias.

\begin{table}[t]

\renewcommand\arraystretch{0.9}


    % \small
    
    \centering
    \setlength{\tabcolsep}{4pt}

    \resizebox{0.9\linewidth}{!}{

    \begin{tabular}{p{1.5cm}|p{3cm}||ccc|ccc}

    \toprule


        \multirow{2}{*}{Dataset} & Explanation? & \multicolumn{3}{c|}{Y}&\multicolumn{3}{c}{N} \\

        \cmidrule{2-8}

         &Temperature&0.1  & 0.5  & 1.0 &0.1  & 0.5  & 1.0    \\

        \midrule

 

        \multirow{5}{*}{BBQ} &\texttt{GPT-3.5-turbo} &46.0 & 46.0 & 46.4 & 42.9 & 43.0 & 40.8   \\ 
        &\texttt{GPT-4o*} &- & - & - & - & - & -   \\
        \cmidrule{2-8}
        &\texttt{Mistral-7b}& 26.9 & 26.9 & 27.0 & 27.2 & 27.4 & 27.3  \\ 
        &\texttt{Llama3-8b} & 24.8 & 23.5 & 23.0 & 25.6 & 27.7 & 26.5  \\ 
       &\texttt{Llama3-70b} & 17.9 & 18.3 & 18.6 & 20.3 & 21.7 & 20.8 \\

        \midrule
        \multirow{5}{*}{DTS}&\texttt{GPT-3.5-turbo} &1.0 & 1.4 & 2.7 & 0.0 & 0.3 & 0.2   \\
        &\texttt{GPT-4o} &27.9 & 26.3 & 25.2 & 0.0 & 0.0 & 0.0   \\
        \cmidrule{2-8}
        &\texttt{Mistral-7b}& 3.7 & 3.8 & 3.3 & 0.7 & 0.7 & 1.3  \\ 
        &\texttt{Llama3-8b} & \textbf{44.6} & 28.7 & 14.4 & \textbf{35.2} & 22.6 & 28.7 \\ 
       &\texttt{Llama3-70b} &  \textbf{70.4} & 63.6 & 43.1 & \textbf{72.8} & 67.0 & 46.3 \\


      \bottomrule

    \end{tabular}

    }

    \caption{Summary of the Bias Rate (\%) with our BiasKG method, varying temperatures.}

    \label{tab:temperature}

\end{table}
    \paragraph{Significance of explanations.} 
    Asking for an explanation has varied effects across different models. For the Llama3 suite of models, the bias rate increases consistently when asked for an explanation, whereas the GPT suite decreases. \texttt{Mistral-7b} has inconsistent results, where bias rate sometimes increases but sometimes decreases. The No Match Rate follows the opposite trend, decreasing in the Llama3 suite of models when asked for an explanation and increasing in the GPT models. We hypothesize asking for reasoning in the Llama3 models increases their tendency to follow instructions, and decreases the efficacy of the safety fine-tuning. In the GPT suite of models, asking for an explanation allows the models to think ``better'' and reduce the bias in their responses.
    
\paragraph{Effect of combining attacks.} We also test combinations of explicit prompting, emotional stimuli, and BiasKG on our open-source datasets, as shown in Table \ref{tab:combos}.
While emotional stimuli does not increase the bias on its own with the BBQ dataset, we find that emotional stimuli combined with direct prompting further increases the bias rate across all open-source models, and decreases the No Match rate for \texttt{Llama3-70b}. It seems that, while the emotional stimuli independently does not contribute to the bias, it can increase the bias rate when used in combination with explicit prompting. The bias rate is further increased when adding BiasKG, although the refusal rate also becomes incredibly high (99\% in \texttt{Llama3-8b}). The best combination is also not consistent across settings (with/without explanation) and models. 



%\vspace{-1mm}
% \subsection{BiasKG} 


    % \paragraph{Efficacy of emotional stimuli depends on the scenario used.}
\begin{figure}[t!]%
  \centering
  \begin{subfigure}[c]{\linewidth}
    \centering
    \includegraphics[trim={1.5cm 5.5cm 0.5cm 12.5cm},clip, width=\linewidth]{figures/bias-identification-experiment-results-KG-chatgpt-gpt-3.5-turbo-csv-setting.png
    }
    % \vspace{0.01cm}
    % \setlength{\belowcaptionskip}{0.05cm}
    % \caption{\texttt{gpt-3.5-turbo}.}
    \label{fig:plotft}
  \end{subfigure}
  \vspace{-0.5mm}
  \begin{subfigure}[c]{\linewidth}
    \centering
    \includegraphics[trim={1.5cm 5.5cm 0.5cm 12.5cm},clip, width=\linewidth]{figures/bias-identification-experiment-results-KG-gpt4-csv-setting.png}
    % \caption{\texttt{gpt-4}.}
  \end{subfigure}
% \vspace{-1.5mm}
  \caption{Deception rate averaged over all temperatures based on prompt template. Top figure is \texttt{gpt-3.5-turbo}, bottom figure depicts \texttt{gpt-4}.}
  \label{fig:plots}
\end{figure}

    \paragraph{Brittleness in efficacy.} Even the latest language models still have inconsistent or unexpected behaviours to our red-teaming attacks. Notably, \texttt{GPT-4o} has very low bias rate (below 1\%) for all settings except specifically the BiasKG method with explanations, where the bias rate suddenly increases to 27.9\%. We further validate this result in Table \ref{tab:temperature}. \texttt{GPT-3.5-turbo} demonstrates low bias rates in its baseline for the DTS dataset, but the bias rate increases to as high as 63\% with emotional stimuli. \texttt{Mistral-7b} exhibits low bias rates for the DTS dataset in every setting except for BiasKG without explanations. There is no notable pattern to this brittleness, which is concerning for potential industry applications. This highlights the importance for further research into LLM safety for safe deployment in production environments.

\subsection{BiasKG Analysis}
    \paragraph{Significance of temperature.} 
    Additionally, we vary the decoding temperature on our BiasKG attack and report results in Table \ref{tab:temperature}. We omit results from \texttt{GPT-4o} on BBQ due to cost considerations, but we did run additional experiments with DTS to validate the outlier result with BiasKG discussed above. For the BBQ dataset, temperature does not have a significant impact on the results, although some results decrease by 1-2\%. The most dramatic results are seen with DTS and the Llama3 models, where the bias rate decreases 17-30\%.

    
We also find the No Match rate is high for some models (eg. \texttt{Llama2-13b}) despite incorporating retries and multiple runs. After manual inspection of the generations, the majority of these errors appear to be \emph{refusals} such as ``I cannot make any assumptions about the individuals based on their background or demographic information...'' The No Match rate generally decreases for the Llama 2 models when we ask for an explanation, indicating the BiasKG effectively bypasses guardrails, but does not necessarily increase the model's bias.



% For the DTS dataset, \texttt{GPT-4} showed a significant rise in deceptive responses from a baseline of 1.4\% to an attacked rate of 14.6\%. 
% The other models did not have enough valid tests related to this dataset to draw reasonable conclusions.

    % \paragraph{Results Across Varied Datasets}
    % We observed different results between the two datasets, BBQ and DTS. BBQ deception rates were much higher overall than DTS. This might be due to the fact that DTS entries are much more explicit in their bias and the safety guardrails that was placed by the creators of each model are working. On the other hand, the bias questioned in the BBQ dataset is much more subtle. Making it much harder for the model to capture.




    
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/kg-similarity.png}
    \caption{The average cosine similarity of the top k entities organized by sensitive attribute.}
    \label{fig:similarity}
\end{figure}
\vspace{-1mm}
    \paragraph{Most Vulnerable Social Groups} We also show the per-attribute Bias Rate (BR) for \texttt{GPT-3.5-turbo} and \texttt{GPT-4} in Figure \ref{fig:plots}. While the weighted BR is low, there are several sensitive attributes with BR above 20\%. We examine the mean cosine similarity among the top $k$ nodes for every sample in BBQ, averaged per sensitive attribute, as a proxy for average stereotype data available. As shown in Figure \ref{fig:similarity}, the cosine similarity varies between 0.74 and 0.78, which is not a significant variation compared to attack effectiveness. This indicates there are certain sensitive attributes tested by BBQ that are more susceptible to our BiasKG attack, independent of the semantic similarity to the contents of our knowledge graph.
\vspace{-1mm}
%     \paragraph{Impact of Temperature}
    
%      We experiment with increasing temperatures across all models, as summarized in Table \ref{tab:temperature}. The effect of temperature varies by model. For \texttt{Llama2-7b} and \texttt{Llama2-13b}, the Deception Rate increases as temperature increases. \texttt{Mistral-7b} has decreasing deception rate as temperature increases, and \texttt{GPT-3.5-turbo} varies by whether or not we ask for an explanation from the model.
%      % , we notice deception rate similarly increases. A higher temperature value can make the model's responses more diverse and unpredictable, thereby promoting biased responses.

% \vspace{-1mm}
    % \paragraph{Significance of Explanation}
    % The explanation component played a critical role in the deception rates. We observed when models were explicitly asked for their reasoning, they generally exhibited higher deception rates compared to where no explanation was requested. The only exception is \texttt{GPT-4}, where the Deception Rate was 1.9\% lower. \texttt{GPT-4}, which has superior reasoning capabilities due to model scaling \cite{kaplan2020scaling}, is able to produce non-biased justifications that provide stronger evidence to resist deception.
    % %This suggests that the explanation evokes a sort of introspective thought process in the model that diminishes its likelihood to provide a deceptive response.
    % % The models deviate in their response to the explanation JSON field: the larger 
    % Asking a smaller model for an explanation, such as \texttt{GPT-3.5} or \texttt{Mistral-7b}, appears to generate biased reasoning, likely because the LLM relies more on the biased knowledge provided.
    
    
    % For the DTS dataset, \texttt{GPT-4} showed a significant rise in deceptive responses from a baseline of 1.4\% to an attacked rate of 14.6\%. 
% The other models did not have enough valid tests related to this dataset to draw reasonable conclusions.

    % \paragraph{Results Across Varied Datasets}
    % We observed different results between the two datasets, BBQ and DTS. BBQ deception rates were much higher overall than DTS. This might be due to the fact that DTS entries are much more explicit in their bias and the safety guardrails that was placed by the creators of each model are working. On the other hand, the bias questioned in the BBQ dataset is much more subtle. Making it much harder for the model to capture.


% \begin{figure}[t!]%
%   \centering
%   \begin{subfigure}[c]{\linewidth}
%     \centering
%     \includegraphics[trim={0.5cm 5.5cm 0.5cm 12.5cm},clip, width=\linewidth]{figures/bias identification - experiment results - KG - chatgpt(gpt-3.5-turbo).csv_setting.png}
%     % %\vspace{0.01cm}
%     % \setlength{\belowcaptionskip}{0.05cm}
%     % \caption{\texttt{gpt-3.5-turbo}.}
%     \label{fig:plotft}
%   \end{subfigure}
%   %\vspace{-0.5mm}
%   \begin{subfigure}[c]{\linewidth}
%     \centering
%     \includegraphics[trim={0.5cm 5.5cm 0.5cm 12.5cm},clip, width=\linewidth]{figures/bias identification - experiment results - KG - gpt4.csv_setting.png}
%     % \caption{\texttt{gpt-4}.}
%   \end{subfigure}
% % %\vspace{-1.5mm}
%   \caption{Deception rate averaged over all temperatures based on prompt template. Top figure is \texttt{gpt-3.5-turbo}, bottom figure depicts \texttt{gpt-4}.}
%   \label{fig:plots}
% \end{figure}


%\vspace{-1mm}
    % \paragraph{Most Vulnerable Social Groups} We also show the per-attribute Deception rate for \texttt{GPT-3.5-turbo} and \texttt{GPT-4} in Figure \ref{fig:plots}. While the weighted deception rate is low, there are several sensitive attributes with deception rates above 20\%.  We report the mean cosine similarity among the top $k$ nodes for every sample in BBQ, averaged by sensitive attribute, as shown in Figure \ref{fig:similarity}. As shown, the cosine similarity does not vary much between attributes, being between 0.74 and 0.78 overall. While inconclusive, we believe this indicates there are stronger safety measures against certain sensitive attributes, irrelevant to the similarity of our BiasKG knowledge.
    
%\vspace{-1mm}
    % \paragraph{Impact of Temperature}
    
     % We experiment with increasing temperatures across all models, as summarized in Table \ref{tab:temperature}. The effect of temperature varies by model. For \texttt{Llama2-7b} and \texttt{Llama2-13b}, the Deception Rate increases as temperature increases. \texttt{Mistral-7b} has decreasing deception rate as temperature increases, and \texttt{GPT-3.5-turbo} varies by whether or not we ask for an explanation from the model.
     % , we notice deception rate similarly increases. A higher temperature value can make the model's responses more diverse and unpredictable, thereby promoting biased responses.

%\vspace{-1mm}
    % The explanation component played a critical role in the deception rates. We observed when models were explicitly asked for their reasoning, they generally exhibited lower deception rates compared to the situation where no explanation was requested (Explanation 'N'). The only exception is \texttt{GPT-4}, where the Deception Rate was 1.9\% higher.
    % This suggests that the explanation evokes a sort of introspective thought process in the model that diminishes its likelihood to provide a deceptive response.
    % The models deviate in their response to the explanation JSON field: the larger 
    % On the other hand, the second behaviour is a drop in the deception rate when there is an explanation. This behaviour is slightly more intuitive as the model has more reasoning evidence to avoid being deceived. The former can be witnessed in the \texttt{GPT-3.5-Turbo} and \texttt{Mistral-7b}, and the latter is found in \texttt{GPT-4} and both \texttt{Llama2} models. 
    % This was discrepancy in behaviours was observed in the BBQ dataset but not in the DTS dataset. Potentially because the BBQ dataset is less direct. The DTS dataset only observed the former behaviour where an explanation increases deception.
    
    % \paragraph{Polarity and Ambiguity}

